Correspondence Distillation from NeRF-based GAN

The neural radiance field (NeRF) has shown promising results in preserving the fine details of objects and scenes. However, unlike mesh-based representations, it remains an open problem to build dense correspondences across different NeRFs of the same category, which is essential in many downstream tasks. The main difficulties of this problem lie in the implicit nature of NeRF and the lack of ground-truth correspondence annotations. In this paper, we show it is possible to bypass these challenges by leveraging the rich semantics and structural priors encapsulated in a pre-trained NeRF-based GAN. Specifically, we exploit such priors from three aspects, namely 1) a dual deformation field that takes latent codes as global structural indicators, 2) a learning objective that regards generator features as geometric-aware local descriptors, and 3) a source of infinite object-specific NeRF samples. Our experiments demonstrate that such priors lead to 3D dense correspondence that is accurate, smooth, and robust. We also show that established dense correspondence across NeRFs can effectively enable many NeRF-based downstream applications such as texture transfer.

==> DDF/experiments/implementation_details.tex <==
% !TEX root = ../main.tex


==> DDF/related_work/not_used_3d_shape_representation.tex <==
\subsection{Neural Implicit Functions (NIFs)}
Recent advances in implicit shape representations \cite{mescheder2019occupancy, park_deepsdf_2019} have demonstrated their excellence when representing complicated geometry.
Though good at approximating individual shapes, 
the implicit nature provides no information about the semantic relationships across shapes, 
unlike in 
mesh \cite{} where vertex-to-vertex correspondences can be easily derived.
To alleviate this limitation, 
Zheng\cite{zheng2021deep} and Deng\cite{deng2021deformed}
proposed to decompose a DeepSDF\cite{park_deepsdf_2019} into a conditioned warping field and a template field shared among the same object category.
Nonetheless, 
these methods still require 3D supervision during training
and are limited to modeling synthetic data.


Neural Implicit Functions were introduced to represent geometry by constructing a continuous volumetric field and 
embedding shapes as its iso-surface \cite{}. 
In recent years, 
implicit functions have been combined with neural networks ~\cite{mescheder2019occupancy,park_deepsdf_2019,chabra_deep_2020,jiang_local_2020}
and show promising results on representing complicated geometry.
For example, 
Sitzmann \etal \cite{sitzmann_scene_2019} show that surfaces of complex scene can be represented by a 5-layer MLP with periodic functions as activation.
Mildenhall \etal~\cite{mildenhall2020nerf} encode scene properties as a continuous function with a well-designed MLP and enable photo-realism volumetric rendering as well as multi-view consistency.  
% deep local shapes
However, parameterize the whole scene with a single MLP needs high-frequency kernels \cite{} as input and hard to encode local details.
Some later studies proposed to blend multiple local implicit functions to generalize to more complex scenes as well as to capture more geometric details\cite{}.
% generality ?
% To overcome the restriction of modeling 
% dynamic
Researchers also try to extend the implicit representations to model dynamic scenes\cite{}, 
though these methods are restricted to overfitting on a short video sequence without large motions.
% dense correspondence
To model dense correspondence between different shapes represented by NIFs, 
\cite{} proposed to formulate NIFs as conditional deformations of an explicit template field parameterized by a MLP or LSTM.
\cite{} solved this problem implicitly by learning a set of semantic part embeddings in the latent space via semantic consistency,
but failed to generalize to arbitrary numbers of parts.

However, %todo
the above mentioned methods need explicit 3D supervision during training and cannot generalize to real-world category,
such as human faces. % carla dataset?
In this work, 
we leverage the insight that GANs internal spatial representations are discriminative enough
to be applied to feature matching and learning robust dense correspondence.  


\subsection{Learning-based 3D reconstruction} % merge into 3D representation
Common approach to address these issues can be categorized in two ways. 
The first category 
learns a prior-based reconstruction module.
\cite{sitzmann_scene_2019} trains a hyper-network to map images to MLP parameters to improve generality. Other works~\cite{mescheder2019occupancy,park_deepsdf_2019,chabra_deep_2020,jiang_local_2020} map a conditional latent code to a single neural network to capture cues of the same class. 
% The first approaches try to alleviate this problem by learning a prior-based reconstruction module, 
% which includes training a hypernetwork to map from partial observations to MLP weights \cite{sitzmann_scene_2019}, 
% or condition latent code to a single neural network to represent signals of the same class\cite{mescheder2019occupancy,park_deepsdf_2019,chabra_deep_2020,jiang_local_2020}. 
Another line of methods treat this problem as an optimization-based meta-learning \cite{tancik_learned_2020,sitzmann_metasdf_2020}, 
learning priors underlying certain classes of signals, achieving both faster convergence and better inference generalization. 
% allowing the network to learn prior behind certain classes of signals and enables both faster convergence and better generalization during test time.
Training time is indeed notoriously long for learning-based methods. For example, recovering high resolution radiance fields with NeRF~\cite{mildenhall2020nerf} and methods alike takes hours and even days.
% Meanwhile, encoding a given signal into network typically requires solving an optimization problem from scratch. 
% For example, recovering a high resolution radiance field, 
% as in NeRF\cite{mildenhall2020nerf}, takes hours even days.

\section{Structured Implicit Representation}
Learning Shape Templates with Structured Implicit Functions

==> DDF/thinking.tex <==
% !TEX root = ../main.tex
Hi\cite{3DCODED}

